Evaluating Factual Consistency of Summaries with Large Language Models

Detecting factual errors in summaries has been an important and challenging subject in summarization research. Inspired by the emergent ability of large language models (LLMs), we explore evaluating factual consistency of summaries by directly prompting LLMs. We present a comprehensive empirical study to assess the ability of LLMs as factual consistency evaluators, which consists of (1) analyzing different LLMs such as the GPT model series and Flan-T5; (2) investigating a variety of prompting methods including vanilla prompting, chain-of-thought prompting, and a sentence-by-sentence prompting method to tackle long summaries; and (3) evaluating on diverse summaries generated by multiple summarization systems, ranging from pre-transformer methods to SOTA pretrained models. Our experiments demonstrate that prompting LLMs is able to outperform the previous best factuality systems in all settings, by up to 12.2 absolute points in terms of the binary classification accuracy on inconsistency detection.

==> related_work.tex <==
\section{Related Work}
\paragraph{Factual consistency evaluation:}
Prior factuality evaluation approaches can be divided into two categories: entailment-based methods and question answering (QA) methods. Entailment-based methods aim to determine whether a summary is entailed by the original document or not. 
%\jhc{This kind of method has an assumption that a summary is either entailed or contains factual incorrectness. So they often use reference summaries as baseline,}
They often apply %\jhc{transformations include both semantically-invariant and semantically-variant on these data to construct a dataset on which could train a classification model}
both semantically-variant and semantically-invariant transformations to the summaries to construct a classification dataset to train the evaluation model~\citep{goodrich2019assessing, kryscinski2020evaluating, goyal2020evaluating, zhao2020reducing}. 
 %\jhc{A crutial design points in these methods are the granularity it focus on. For instance, xxx has proposed quantity entailment method concentrating on the quantity correctness, xx has introduced the dependency parsing-entailment by evaluating the dependency arcs in the summary. These methods have two main drawbacks. 1. As mentioned in FactCC, the transformations applied by the authors cannot contain all kinds of factual inconsistencies occurred in summarization task, making the results limited 2. There is no commonsense for the defination of entailment, therefore we cannot say entailment is equal to faithfulness.}
 Relying on heuristic transformations cannot cover all types of factual errors in summarization, limiting its performance as mentioned in~\citet{kryscinski2020evaluating}.
 %\jhc{you cannot say entailment is not equal to faithfulness since we are casting faithfulness as an entailment task} 
%\jhc{The second type of method}
On the other hand, QA-based methods automatically yield questions to probe the facts in the document or summary, and then assess whether the facts in the document and the summary are consistent by answering these questions~\citep{wang2020asking,durmus2020feqa,scialom2021questeval} 
% follow three steps: (1) generate relevant questions; (2) answer these questions with either the document or the summary separately; and (3) compare the answers to assess whether they are consistent.
% \jh{Not sure if all the QA related work follow these 3 steps, maybe we should further clarify}
%  \jhc{is originated from the intuition that we can ask questions to both the summary and the document. Then we can compare the answers.}{ask questions about the facts in the summary and try to find answers from the document to verify the facts~\citep{xxx}.} \jhc{This method follows three steps: 1. question generation. 2. question answer with both the document and the summary. 3. Compare the similarity score of the answers from the second step. Following works concentrate on the balance between the precise and recall. xxx }{}
%\jhc{The drawback of this kind of method is that it}
These approaches need %\jhc{a lot of}
to train several additional models %\jhc{to be trained}{} 
%\jhc{including}
for question generation, question answering, or answer comparison,
%\jhc{, and comparing model separately}{}
 %\jhc{is time-consuming and data source consuming}
where corresponding annotations are required and the errors of intermediate components could propagate to the final predictions.  
% \jh{I removed the related work discussion on datasets -- a short description of exising datasets could appear in our datasets selection section}
% \subsection{Factual correctness evaluation} 
% All the methods discussed above require a dataset to evaluate the performance of the proposed metric, and these authors hold the hypothesis that human annotators have the best judgment capability. As a result, these authors label the summaries manually by the authors themselves or by hiring crowd-source or trained annotators to give judgments.

% The granularity of the labels are diverse, from summary based(xx ) to sentence based or more finer-grained such as phrase based and word based.

% Aggrefact\citep{tang2022understanding}, which is recent research, takes the timeliness of the language model that generates the summaries into account. Based on this insight, the authors separate the data into three classes: Sota, Former and Old. Sota consists of state-of-the-art summarization models including BART, PEGASUS, and T5. FORMER collects early Transformer-based summarization models including BERTSum and GPT-2. The remaining models are older models such as Pointer generator and BottomUp. The authors discover the exsiting factuality systems act worse on the SOTA data than on the former/old data by evaluating exsiting evaluation systems on this new benchmark. This finding provides us insight that the evaluation systems need to be updated considering the summarization model's progress. 


\paragraph{Prompt-based learning:}
% \citet{brown2020language} has brought few-shot prompting into people's attention. Prompt learning gives us a general method to better use the ability of large language models. By designing a good prompt indicating our demand, you can use the large language model to do a variety of tasks. Although Large language models have shown surprising understanding and expression ability on some common tasks such as translation, classification, QA or so. Nonetheless, they still struggle with some more complicated tasks. That's why there is still gap between big models and real artificial intelligence. Chain of thought prompting provides a possible solution to fill this gap.
Prompts in the context of language models refer to text instructions concatenated with the test input (zero-shot) or with few exemplars and the test input (few-shot). 
Large language models are able to perform various tasks without tuning~\citep{radford2019language,brown2020language,liu2021pre} when the prompts are fed into as the input to signal the task. 
Instruction tuning futher lifts the ability of LLMs to follow instructions in the prompts~\citep{wei2022finetuned,sanh2022multitask,ouyang2022training,chung2022scaling,iyer2022opt}. 
Recently, chain-of-thought prompting is proposed to trigger the reasoning abilities of LLMs, by asking the model to explain the thinking process during generation~\citep{kojima2022large,wei2022chain}.
% Since then, several following work are presented to futher improve the reasoning performance of LLMs, including self-consistency decoding~\citep{wang2022self}, least-to-most prompting~\citep{zhou2022least}, and reasoning with self-verification~\citep{weng2022large}.
In addition to text prompts,~\citet{gao2022pal} and~\citet{chen2022program} introduce program-of-thought prompting to generate executable code to perform numerical reasoning tasks. 
% \subsection{Chain of Thought prompting}
%  Chain of thought prompting approach is proposed by Jason. By showing a few helpful exemplars containing the reasoning steps and adding instructions such as "Let's think step by step" in the instruction, we can render the language model to generate logical and well-organized content. This approach is extremely helpful for tasks on high-demand reasoning tasks. Some other strategies are proposed based on cot. For instance, least-2-most prompting generates sub-questions in the first step to facilitate the reasoning process and answers these subquestions then. Self-consistency voting proposed by Wang is to select the best final results by sampling multiple times. The intuition of dividing complex reasoning problems into easier tasks and conquering them one by one behind the cot-based prompting is remarkably inspiring to solve reasoning problems.
